A new method to find out the optimal neutron moderator size based on neutron scattering instrument parameters

Simple and fast analytic method to find out optimal combinations of sizes of neutron moderator and optical system entrance, allowing for the full sample illumination with minimum to none background, is developed. In the case of employing low-dimensional para-hydrogen moderators with enhanced neutron beam brilliance, the method allows to determine the minimum size of moderator, which provides the highest sample flux while keeping the sample fully illuminated. This method can be used during the design of new neutron sources, upgrades of neutron optical systems and moderator replacements.

==> parameters.tex <==
\subsection{Choice of instrument parameters}
\label{parameters}
add here about $n$

Finally, consider an instrument with parameters $d_s$ and $\alpha_s$ not fixed. Reducing one of them allows to optimally use smaller moderator with higher brilliance. However, the PS volume $V_s$ is reduced, thus it is not clear what happens to total number of neutrons at the sample.

We now consider NF-NF type NTS with double-slit collimation and $n=2$. For each combination of $d_s$ and $\alpha_s$ one can find COFSI minimum according to Eqs.~(\ref{w_min1}--\ref{w_min}) and (\ref{D_min}). Then one calculates brilliance corresponding to the moderator size using function shown in Fig.~\ref{ph2}. Taking into account Eqs.~(\ref{sample_flux_eq}) and (\ref{sample_volume}) one finds maximal sample flux.

\begin{figure}[h!]
\begin{center}
\begin{minipage}[h]{0.47\linewidth}
\centering
\includegraphics[width=1\linewidth]{sample_scan_nff.eps} \\ (a)

\end{minipage}
\begin{minipage}[h]{0.47\linewidth}
\centering
\includegraphics[width=1\linewidth]{sample_scan_nfnf.eps} \\ (b)

\end{minipage}
\caption{Sample flux for different combinations of sample size $d_s$ and required collimation $\alpha_s$.}
\label{sample_scan}
\end{center}
\end{figure}

Fig.~\ref{sample_scan}a shows sample flux in case of NF-F NTS with $L_{in}=2000$~mm. This case corresponds e.g. to reflectometer's focusing plane. Smaller collimation or sample size always lead to reduced sample flux. Thanks to high brilliance of para-H$_2$ this flux is higher than one could expect from simple proportion: instrument with $d_s=100$~mm and $\alpha_s=2$\textdegree{} has sample flux of 3; instrument with reduced $\alpha_s=0.5$\textdegree{} has sample flux of 1.5 (not 0.75); instrument with reduced $d_s=10$~mm has sample flux of 0.8 (not 0.3).

Next we consider NF-NF NTS with double-slit collimation and $n=2$, that corresponds to e.g. reflectometers's scattering plane. Sample flux in this case is shown in Fig.~\ref{sample_scan}b. Too large sample size or too relaxed angular resolution leads to reduced sample flux. The moderator size becomes too large and provide too low brilliance. In other words, for a particular sample size there is particular collimation $\alpha_s$, providing highest possible sample flux. Similarly, for any given resolution $\alpha_s$ there is sample size corresponding to highest possible sample flux.

Creating and analysing sample flux maps like in Fig.~\ref{sample_scan} is useful for refinement of instrument requirements if they are not too strictly defined.

DIVIDE DEUTERIUM BY PARAH2 TO BUILD LARGE DIAGRAM DETERMINING WHICH IS BETTER
